Fingerprinting New Physics with Effective Field Theories

Given the absence of direct evidence for new resonances beyond the Standard Model (BSM) at the Large Hadron Collider (LHC) so far, a complementary strategy to search for new physics in an indirect way is provided by the Standard Model Effective Field Theory (SMEFT). As the low-energy limit of a generic ultraviolet (UV) completion of the SM, the SMEFT provides a powerful theoretical framework to correlate deviations from the SM between different processes, offering experimental sensitivity to a plethora of SM extensions. This thesis presents a state-of-the-art SMEFT interpretation of the top, Higgs, diboson and electroweak sectors, taking into account data collected at the Large Electron-Positron Collider (LEP), the SLAC Large Detector (SLD) and the LHC. We also include the effect of the upcoming High-Luminosity LHC (HL-LHC) upgrade and demonstrate the unprecedented impact on the SMEFT parameter space of two proposed electron-positron colliders: the electron-positron Future Circular Collider (FCC-ee) and the Circular Electron Positron Collider (CEPC). We present constraints both in terms of Wilson coefficients, and couplings and masses of a wide range of UV-complete models through a newly developed automatised limit-setting procedure. We further present novel methodological advances through the development of unbinned multivariate likelihoods specialised to the SMEFT that provide maximal sensitivity to new physics using classification and regression techniques from Machine Learning. Our results provide an extensive characterisation of the SMEFT parameter space as probed both by current and future colliders, providing timely input to the upcoming European Strategy for Particle Physics Update.

==> _inputs/ML4EFT/flowchart.tex <==

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=0.5cm,text centered, draw=black, fill=red!30]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{process} = [rectangle, minimum width=4cm, minimum height=1cm, text centered, draw=black, fill=orange!30, rounded corners, text width=4cm]

% \begin{equation} gin{tikzpicture}[node distance=2cm]
% \node (start) [startstop] {Start};
% \node (in1) [io, below of=start] {Input};
% \node (pro1) [process, below of=in1] {Process 1};
% \node (dec1) [decision, below of=pro1, yshift=-0.5cm] {Decision 1};
% \node (pro2a) [process, below of=dec1, yshift=-0.5cm] {Process 2a text text text text text text text text text text};
% \node (pro2b) [process, right of=dec1, xshift=2cm] {Process 2b};
% \node (out1) [io, below of=pro2a] {Output};
% \node (stop) [startstop, below of=out1] {Stop};
% \draw [arrow] (start) -- (in1);
% \draw [arrow] (in1) -- (pro1);
% \draw [arrow] (pro1) -- (dec1);
% \draw [arrow] (dec1) -- (pro2a);
% \draw [arrow] (dec1) -- (pro2b);

% \draw [arrow] (dec1) -- node[anchor=east] {yes} (pro2a);
% \draw [arrow] (dec1) -- node[anchor=south] {no} (pro2b);
% \draw [arrow] (pro2b) |- (pro1);
% \draw [arrow] (pro2a) -- (out1);
% \draw [arrow] (out1) -- (stop);
% \end{tikzpicture}
\begin{equation} gin{figure}[htbp]
\small
    \centering
    \begin{equation} gin{tikzpicture}[node distance=2cm]

\node (in1) [io] {\verb|smeftsim_main.fr|};
\node (pro1) [process, below of=in1] {\verb|SMEFTsim| \verb|Flavour = topU3l|, \verb|Scheme=MwScheme|};
\node (out1) [io, below left=of pro1] {\verb|FeynArts .mod file|};
\node (out2) [io, below right=of pro1] {\verb|FeynArts .gen file|};
\node (pro2a) [process, below of=pro1, node distance=6cm] {\verb|FeynArts|: draw topologies and insert fields};
\node (pro2b) [process, below of=pro2a] {\verb|FormCalc|: compute $\left|\mathcal{M}_{\mathrm{sm}} + \mathcal{M}_{\mathrm{eft}}(\boldsymbol{c})\right|^2$};
\node (pro2c) [process, below of=pro2b] {\verb|Mathematica|: compute $d\sigma(\boldsymbol{c})$};
\node (out3) [io, below of=pro2c] {Analytical $d\sigma(\boldsymbol{c})$};
% \node (out1) [io, below of=pro2a] {Output};
% \node (stop) [startstop, below of=out1] {Stop};

\draw [arrow] (in1) -- (pro1);
% \draw [arrow] (pro1) -- (dec1);
% \draw [arrow] (dec1) -- (pro2a);
% \draw [arrow] (dec1) -- (pro2b);

% \draw [arrow] (dec1) -- node[anchor=east] {yes} (pro2a);
% \draw [arrow] (dec1) -- node[anchor=south] {no} (pro2b);
\draw [arrow] (pro1) -| (out1);
\draw [arrow] (pro1) -| (out2);
\draw [arrow] (out1) |- (pro2a);
\draw [arrow] (out2) |- (pro2a);
\draw [arrow] (pro2a) -- (pro2b);
\draw [arrow] (pro2b) -- (pro2c);
\draw [arrow] (pro2c) -- (out3);
% \draw [arrow] (pro2a) -- (out1);
% \draw [arrow] (out1) -- (stop);
\end{tikzpicture}
    \caption{Flow diagram indicating the pipeline adopted
    in this work to evaluate analytical expressions
    of differential distributions in the SMEFT for
    the LHC processes considered.
    %
    These analytical cross-section are evaluated at leading order
    and at the parton level, where they are compared
    with numerical simulations
    for the same theoretical settings.
    %
    The analytical cross-section provide access to the
    exact likelihood ratio, which in turn makes possible a reference
    benchmark for the performance of the ML algorithm.
    }
    \label{fig:pipeline_flowchart}
\end{figure}


==> _inputs/ML4EFT/tables/fisher_tt_inclusive.tex <==
\begin{equation} gin{table}[htbp]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.50}
\begin{equation} gin{tabular}{|c|c|c|c|}
\hline
 \multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Processes} \\ \hline
 Class & Coefficient & $t\bar{t}$ (8 TeV) & $t\bar{t}$ (13 TeV) \\ \hline
\multirow{14}{*}{2L2H}
 & {\color{blue}$c_{qq}^{1,8}$} & { \color{black} 1.003}({\color{black} -0.260}) & { \color{black} 2.710}({\color{black} 1.923})\\ \cline{2-4} 
 & $c_{qq}^{1,1}$ & { \color{black} 0.000}({\color{black} -4.743}) & { \color{black} 0.000}({\color{black} 7.211})\\ \cline{2-4} 
 & $c_{qq}^{8,3}$ & { \color{black} 0.086}({\color{black} -1.006}) & { \color{black} 0.157}({\color{black} 2.164})\\ \cline{2-4} 
 & $c_{qq}^{1,3}$ & { \color{black} 0.000}({\color{black} -4.788}) & { \color{black} 0.000}({\color{black} 7.384})\\ \cline{2-4} 
 & {\color{blue}$c_{qt}^{8}$} & { \color{black} 0.997}({\color{black} -0.294}) & { \color{black} 2.802}({\color{black} 2.185})\\ \cline{2-4} 
 & $c_{qt}^{1}$ & { \color{black} 0.000}({\color{black} -4.929}) & { \color{black} 0.000}({\color{black} 6.670})\\ \cline{2-4} 
 & {\color{blue}$c_{ut}^{8}$} & { \color{black} 0.414}({\color{black} -0.305}) & { \color{black} 1.097}({\color{black} 1.146})\\ \cline{2-4} 
 & $c_{ut}^{1}$ & { \color{black} 0.000}({\color{black} -3.229}) & { \color{black} 0.000}({\color{black} 4.280})\\ \cline{2-4} 
 & {\color{blue}$c_{qu}^{8}$} & { \color{black} 0.411}({\color{black} -0.321}) & { \color{black} 1.187}({\color{black} 1.174})\\ \cline{2-4} 
 & $c_{qu}^{1}$ & { \color{black} 0.000}({\color{black} -3.193}) & { \color{black} 0.000}({\color{black} 4.251})\\ \cline{2-4} 
 & {\color{blue}$c_{dt}^{8}$} & { \color{black} 0.132}({\color{black} -0.301}) & { \color{black} 0.353}({\color{black} 0.888})\\ \cline{2-4} 
 & $c_{dt}^{1}$ & { \color{black} 0.000}({\color{black} -1.753}) & { \color{black} 0.000}({\color{black} 2.328})\\ \cline{2-4} 
 & {\color{blue}$c_{qd}^{8}$} & { \color{black} 0.129}({\color{black} -0.313}) & { \color{black} 0.355}({\color{black} 0.901})\\ \cline{2-4} 
 & $c_{qd}^{1}$ & { \color{black} 0.000}({\color{black} -1.768}) & { \color{black} 0.000}({\color{black} 2.347})\\ \hline
\multirow{1}{*}{2FB}
 & {\color{blue}$c_{tG}$} & { \color{black} 96.829}({\color{black} 127.204}) & { \color{black} 91.339}({\color{black} 55.149})\\ \hline
\end{tabular}
\vspace*{5mm}
\caption{The normalised Fisher information for $t\bar{t}$ inclusive production at 8 TeV (left) and 13 TeV (right) grouped by operator class. We show results both at the linear level as well as the quadratic level in the EFT expansion, where the latter are given in parenthesis.}
\label{eq:fisher_tt_inclusive}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> _inputs/ML4EFT/tables/fisher_vh.tex <==
\begin{equation} gin{table}[H]
\footnotesize
\centering
\begin{equation} gin{tabular}{|c|c|c|}
\hline
 Class & Coefficient &  \href{https://arxiv.org/abs/1903.04618}{${\rm ATLAS\_ZH\_Hbb\_13TeV}$} \\ \hline
\multirow{14}{*}{2L2H}
 & $c_{qq}^{1,8}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qq}^{1,1}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qq}^{8,3}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qq}^{1,3}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qt}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qt}^{1}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{ut}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{ut}^{1}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{qu}^{8}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qu}^{1}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{dt}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{dt}^{1}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qd}^{8}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{qd}^{1}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \hline
\multirow{10}{*}{2FB}
 & $c_{t \varphi}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{tG}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{b \varphi}$ & { \color{blue} 0.000}({\color{blue} 0.000})\\ \cline{2-3}
 & $c_{c \varphi}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{\tau \varphi}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3} 
 & $c_{tW}$ & { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{tZ}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{\varphi Q}^{3}$ & { \color{black} 0.007}({\color{black} 1.980})\\\cline{2-3}
 & $c_{\varphi Q}^{(-)}$ & { \color{black} 0.002}({\color{black} 3.031})\\ \cline{2-3} 
 & $c_{\varphi t}$ &  { \color{black} 0.000}({\color{black} 0.000})\\ \hline
\multirow{6}{*}{B}
 & $c_{\varphi G}$ &{ \color{black} 0.000}({\color{black} 0.000})\\ \cline{2-3}
 & $c_{\varphi B}$ & { \color{blue} 0.006}({\color{blue} 0.001})\\ \cline{2-3}
 & $c_{\varphi W}$ &  { \color{blue} 0.423}({\color{blue} 16.162})\\ \cline{2-3} 
 & $c_{\varphi WB}$ &  { \color{blue} 84.717}({\color{blue} 25.306})\\ \cline{2-3}
 & $c_{\varphi d}$ & { \color{blue} 0.008}({\color{blue} 0.028})\\ \cline{2-3}
 & $c_{\varphi D}$ &{ \color{blue} 14.838}({\color{blue} 53.492})\\ \hline
\end{tabular}
	\caption{The normalised Fisher information for $ZH$ production, $Z\rightarrow \ell \ell$, $H \rightarrow b \bar{b}$ at 13 TeV grouped by operator class. We show results both at the linear level as well as the quadratic level in the EFT expansion, where the latter are given in parenthesis. {\color{red} update $c_{b\varphi}$}\label{tab:fisher_vh}}
\end{table}


==> _inputs/smefit3/app-benchmarking.tex <==
\section{EWPOs implementation: benchmarking and validation}
\label{app-benchmarking}

Our implementation of EWPOs in {\sc\small SMEFiT}, described in Sect.~\ref{sec:ewpos}, has been cross-checked and validated with previous studies, in particular with the analysis of~\cite{Brivio:2017bnu}. 
%
To highlight the consistency of our implementation with previous results, we provide in Fig.~\ref{fig:ew-benchmark-comp} a comparison of single parameter fits at linear order in the EFT  carried out with {\sc\small SMEFiT} with the EWPO data in Table~\ref{tab:ew-datasets}
against the corresponding analysis from~\cite{Brivio:2017bnu}
based on the same dataset and assuming flavour universality for comparison purposes.
 %
The triple gauge operator $O_{WWW}$ differs from the SMEFT@NLO convention by a minus sign to adopt the same conventions as~\cite{Brivio:2017bnu}, and has been fitted to the same subset of the available LEP data on $WW$ production composed of only 4 bins.
%
Excellent agreement is found for all operators, further validating the implementation of EWPOs presented in this work.

%-----------------------------
\begin{figure}[t]
\centering\includegraphics[width=0.90\linewidth]{_inputs/smefit3/figures/ewpo_benchmark.pdf}
    \caption{Comparison of a {\sc\small SMEFiT}-based analysis
of the EWPOs from LEP against the corresponding analysis from~\cite{Brivio:2017bnu}.
%
We display bounds at the $68\%$ CL for one-parameter fits using linear EFT and LO calculations.
%
One should note that we adopt the convention of~\cite{Brivio:2017bnu} for the
triple gauge operator $O_{WWW}$, which differs from the SMEFT@NLO one by a negative sign. 
%
For consistency with the settings
adopted in~\cite{Brivio:2017bnu}, the triple
gauge operator coefficient $c_{WWW}$ has been fitted to a subset
of the available LEP data on diboson production composed by only 4 bins.}
    \label{fig:ew-benchmark-comp}
\end{figure}
%------------------------


==> _inputs/smefit_uv/app-UV_details.tex <==

%\subsection{Tree-level matched one-particle models}
\label{app:uv_model_details}

In this appendix we provide complementary
information on the UV-complete scenarios
studied in this work, in particular concerning
the tree-level matched one-particle models.

For each of the one-particle
UV models considered here
and listed in Table~\ref{tab:UV_particles},
we indicate the relevant couplings
entering their Lagrangian in
Table~\ref{tab:uv_couplings_SMEFiT},
where as elsewhere in the paper
we follow the notation from~\cite{deBlas:2017xtg}.
%
These are the UV parameters 
which are constrained from 
the data via the matching procedure.
%
 These couplings have been selected such that the resulting
 Wilson coefficients at the matching scale fulfil the \smefit~flavour assumptions
 in the case of tree-level matching.
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\renewcommand{\arraystretch}{1.5}
\begin{center}
\begin{tabular}{c|c||c|c||c|c}
\multicolumn{2}{c||}{\bf Scalars} & \multicolumn{2}{c||}{\bf Fermions} & \multicolumn{2}{c}{\bf Vectors} \\
\midrule
Model & UV couplings & Model & UV couplings & Model & UV couplings \\
\hline
$\mathcal{S}$ & $\kappa_{\mathcal{S}}$ & $N$ & $\left(\lambda_N^e\right)_3$ & $\mathcal{B}$ & $\left(g_B^u\right)_{33}$, $\left(g_B^q\right)_{33}$, $g_B^\varphi$, \\
 $\phi$       & $\lambda_{\phi},\,\, (y_{\phi}^u)_{33}$ & $E$ & $\left(\lambda_E\right)_3$ & & $\left(g_B^e\right)_{11}$, $\left(g_B^e\right)_{22}$, $\left(g_B^e\right)_{33}$,  \\
$\Xi$  & $\kappa_{\Xi}$ & $\Delta_1$ & $\left(\lambda_{\Delta_1}\right)_3$ & & $\left(g_B^\ell\right)_{22}$, $\left(g_B^\ell \right)_{33}$ \\
$\Xi_1$ & $\kappa_{\Xi_1}$ & $\Delta_3$ & $\left(\lambda_{\Delta_3}\right)_3$ & $\mathcal{B}_1$ & $g_{B_1}^\varphi$  \\
$\omega_1$ & $\left(y_{\omega_1}^{qq}\right)_{33}$ & $\Sigma$ & $\left(\lambda_{\Sigma}\right)_3$ & $\mathcal{W}$ &  $\left(g_{\mathcal{W}}^l\right)_{11} = 2\,\left(g_{\mathcal{W}}^l\right)_{22}$, $\left(g_{\mathcal{W}}^l\right)_{33}$ \\
$\omega_4$ & $\left(y_{\omega_4}^{uu}\right)_{33}$ & $\Sigma_1$ & $\left(\lambda_{\Sigma_1}\right)_3$ & & $g_{\mathcal{W}}^\varphi$, $\left(g_{\mathcal{W}}^q\right)_{33}$  \\
$\zeta$ & $\left( y_{\zeta}^{qq} \right)_{33}$ & $U$ & $\left(\lambda_{U}\right)_3$ & $\mathcal{W}_1$ & $g_{\mathcal{W}_1}^\varphi$ \\
$\Omega_1$ & $\left(y_{\Omega_1}^{qq}\right)_{33}$ & $D$ & $\left(\lambda_{D}\right)_3$ & $\mathcal{G}$ &  $\left(g_{\mathcal{G}}^q \right)_{33}$, $\left(g_{\mathcal{G}}^u\right)_{33}$ \\
$\Omega_4$ & $\left(y_{\Omega_4}\right)_{33}$ & $Q_1$ & $\left(\lambda_{\mathcal{Q}_1}^u\right)_3$ &  &  \\
$\Upsilon$ & $\left(y_{\Upsilon}\right)_{33}$ & $Q_7$ & $\left(\lambda_{\mathcal{Q}_7}\right)_3$ &  $\mathcal{H}$ & $\left(g_{\mathcal{H}}\right)_{33}$ \\
$\Phi$ & $\left(y_{\Phi}^{qu}\right)_{33}$ & $T_1$ & $\left(\lambda_{T_1}\right)_3$ &  $\mathcal{Q}_5$ & $\left(g_{\mathcal{Q}_5}^{uq}\right)_{33}$ \\
  &   & $T_2$ & $\left(\lambda_{T_2}\right)_3$ & $\mathcal{Y}_5$ & $\left(g_{\mathcal{Y}_5}\right)_{33}$ \\
\bottomrule
\end{tabular}
\caption{\label{tab:uv_couplings_SMEFiT} For each of the one-particle
UV models considered in this work
and described in Table~\ref{tab:UV_particles},
we list the couplings
entering their Lagrangian,
restricting ourselves to those which are consistent with the {\sc\small SMEFiT} flavour assumption after tree-level matching.
}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

It is worth noting that in most models
considered, the interaction with the top quark is singled out and treated differently from the lighter quarks, consistently
with the {\sc\small SMEFiT} assumptions.
%
This is a well-motivated assumption and is realised in many common UV scenarios, such as in partial compositeness. 
%
Concerning the leptonic sector, 
the {\sc\small SMEFiT} flavour assumption allows for independent couplings to the different generations. 

This situation differs from the models considered by the {\sc\small FitMaker} collaboration~\cite{Ellis:2020unq}, in which the same heavy particles are used but the couplings are assumed to be flavour-universal.
%
For the case of heavy spin-one bosons, they assume couplings only to the Higgs boson where appropriate. 
%
The {\sc\small FitMaker} models $BB_1$ and $Q_{17}$ arise by considering the pairs of heavy particles $\lbrace \mathcal{B}, \mathcal{B}_1 \rbrace$ and $\lbrace Q_1, Q_7 \rbrace$ respectively, with degenerate masses and couplings. 
%
The models $T$ and $TB$ contain the heavy fermions $U$ and $Q_1$ respectively with specially rescaled couplings~\cite{Dawson:2020oco}.

Table~\ref{tab:Fitmaker_models_flavour} indicates, for the UV models
 considered in the {\sc\small FitMaker}
 study~\cite{Ellis:2020unq} and which are compared
 with our results
 in Fig.~\ref{fig:fitmaker_vs_smefit_all},
  whether they comply 
 with the flavour symmetry assumed in {\sc\small SMEFiT}, and if
 this is not the case what are the differences.
 %
 Here ``more restrictive than {\sc\small SMEFiT}'' means that applying the {\sc\small SMEFiT} flavour symmetry induces more non-vanishing UV couplings than in the {\sc\small FitMaker} case.
%
For the purposes of the benchmark
comparison of Fig.~\ref{fig:fitmaker_vs_smefit_all}, the effect of 
these additional symmetry-breaking Wilson coefficients has been ignored.
 

%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
	\centering
 \renewcommand{\arraystretch}{1.5}
	\begin{tabular}{c|c|c}
		$\quad\quad$ Model
  $\quad\quad$& $\quad\quad$ Compliant $\quad\quad$ & Details\tabularnewline
		\midrule
		$\mathcal{S}\, (S)$ & Yes & - \tabularnewline
%		\hline
%		$\mathcal{S}_1\,(S_1)$ & No &  $(c_{\ell\ell})_{1111}\neq (c_{\ell\ell})_{1221}$ \tabularnewline
		\hline
		$\phi$  & No &  $(c_{ledq})_{3333}\neq0$, $(c_{quqd})_{3333}\neq0$, $(c_{lequ})_{3333}\neq0$\tabularnewline
		\hline
		$\Xi$ & Yes & - \tabularnewline
		\hline
		$\Xi_1$ & Yes & - \tabularnewline
		\hline
		$\mathcal{B}\,(B)$ & Yes & More restrictive than {\sc\small SMEFiT}\tabularnewline
		\hline
		$\mathcal{B}_1\,(B_1)$ & Yes & - \tabularnewline
		\hline
		$\mathcal{W}\,(W)$ & Yes & More restrictive than {\sc\small SMEFiT} \tabularnewline
		\hline
		$\mathcal{W}_1\,(W_1)$ & Yes & More restrictive than {\sc\small SMEFiT}\tabularnewline
		\hline
		$N$ & No & $(c_{\varphi l}^{(1),(3)})_{ij} \neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$E$ & No & $(c_{\varphi l}^{(1),(3)})_{ij} \neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$T$ & Yes & - \tabularnewline
		\hline
		$\Delta_1$ & No & $(c_{\varphi e})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$\Delta_3$ & No & $(c_{\varphi e})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$\Sigma$ & No & $(c_{\varphi l}^{(1),(3)})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$\Sigma_1$ & No & $(c_{\varphi l}^{(1),(3)})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$U$ & No & $(c_{\varphi q}^{(1),(3)})_{ij}\neq 0$ and $(c_{u\varphi})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$D$ & No & $(c_{\varphi q}^{(1),(3)})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$Q_5$ & No & $(c_{\varphi d})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$Q_7$ & No & $(c_{\varphi u,\,u\varphi})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$T_1$ & No & $(c_{\varphi q}^{(1),(3)})_{ij}\neq 0$ and $(c_{u\varphi})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
		$T_2$ & No & $(c_{\varphi q}^{(1),(3)})_{ij}\neq 0$ and $(c_{u\varphi})_{ij}\neq 0$ for $i\neq j$ \tabularnewline
		\hline
        $U\,(T)$ & Yes & - \tabularnewline
        \hline
		$Q_1\,(TB)$ & No & $(c_{\varphi d})_{33}\neq (c_{\varphi d})_{11,22}$ and $(c_{\varphi ud})_{33}\neq 0$ \tabularnewline
        \hline
        $Q_{17}\,(\lbrace Q_1,\,Q_7 \rbrace)$  & Yes & - \tabularnewline
        \hline
        $BB_{1}\,(\lbrace B,\,B_1 \rbrace)$  & Yes & - \tabularnewline
  \bottomrule
	\end{tabular}
	\caption{For the UV models
 considered in the {\sc\small FitMaker}
 study and which are compared
 with the results of our analysis
 in Fig.~\ref{fig:fitmaker_vs_smefit_all},
 we indicate whether they comply 
 with the flavour symmetry assumed in {\sc\small SMEFiT}, and if
 this is not the case what are the differences.
 %
 Here ``more restrictive than {\sc\small SMEFiT}'' means that applying the {\sc\small SMEFiT} flavour symmetry induces more non-vanishing UV couplings.
 %
 We denote UV models
 following the notation of~\cite{deBlas:2017xtg}
 and 
    we indicate the choice in {\sc\small FitMaker} between parenthesis whenever different.
 %
 The only model for which we use
 a different notation from~\cite{deBlas:2017xtg} is the scalar doublet model $\phi$. }
	\label{tab:Fitmaker_models_flavour}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> _inputs/smefit_uv/app-ewpos.tex <==
\section{Baseline SMEFiT global analysis}
\label{app:ewpos}

The {\sc\small SMEFiT} framework provides a flexible and robust open-source tool to constrain the SMEFT
parameter space using the information provided by experimental data from energy-frontier particle
colliders such as the LHC as well as from
lower-energy experiments.

 Given a statistical model defined by a likelihood
 $L(\boldsymbol{c})$, depending on  parameters $\boldsymbol{c}$ specifying the 
 theoretical predictions 
 for the observables entering the fit, and the
 corresponding dataset $\mathcal{D}$, {\sc\small SMEFiT}  infers the posterior distribution $P(\boldsymbol{c}|\mathcal{D})$ by means
 of sampling techniques~\cite{Feroz:2013hea, Feroz:2007kg}.
%
 {\sc\small SMEFiT} supports the inclusion of quadratic EFT corrections, can work up to NLO precision in the QCD expansion,
 admits general user-defined flavour assumptions and theoretical restrictions, and does
 not have limitations on the number or type of dim-6 operators that can be considered.

Theoretical restrictions on the EFT parameter space can be imposed as follows.
%
Given a set of $N$ fit coefficients $\{c_1,\dots, c_N\}$,
{\sc\small SMEFiT} allows the user to impose relations of the general form,
\begin{equation}
\label{eq:constraints_coeffs_app}
\sum_{i} a_i \lp c_1\rp ^{n_{1,i}} \dots \lp c_N\rp ^{n_{N,i}}=0 \, ,
\end{equation}
where the sum runs over all the possible combinations of the coefficients and $n_{j,i}$ are real numbers such that $\sum_{j} n_{j,i}$ is equal to a constant to preserve the correct dimensionality for all $i$. 
%
For instance, the relationship between the
Wilson coefficients in Eq.~(\ref{eq:rel_UV_tree_2}) arising from the 
heavy scalar model matched at tree-level can be
rewritten in the same format as Eq.~(\ref{eq:constraints_coeffs_app}), namely
\begin{equation}
\label{eq:constraints_coeffs_app_2}
\lp c_{qd}^{(1)}\rp_{3333} \lp \lp c_{u\varphi}\rp_{33} \rp^2   - \lp c_{qu}^{(1)} \rp _{3333}  \lp  \lp c_{d\varphi}\rp_{33} \rp^2  = 0
\end{equation}
These relations have to be imposed on a case-by-case basis via a run card and the user must declare which are the independent coefficients to be fitted. 
%
This functionality can be used to either relate the fit parameters among them,
as in Eq.~(\ref{eq:constraints_coeffs_app_2}), or to perform a mapping to a different
set of degrees of freedom.
%
The latter feature allows one to perform with {\sc\small SMEFiT} the fits on the UV model parameters as presented in this work.

As mentioned in Sect.~\ref{sec:smefit}, in comparison to~\cite{Giani:2023gfq}, which in turn updates the global SMEFT analysis
of Higgs, top quark, and diboson data presented in~\cite{Ethier:2021bye}, here we 
implement in {\sc\small SMEFiT} the information provided by the legacy electroweak
precision observables (EWPOs) from LEP and SLAC~\cite{ALEPH:2005ab} in an exact manner.
%
Previously, the constraints provided by these EWPOs in the SMEFT parameter space were accounted in an approximate manner, assuming EWPOs were measured with vanishing uncertainties.
%
This assumption introduced additional relations between a subset of the Wilson coefficients.
%
While such approximation served the purposes of interpreting LHC measurements, it is not appropriate
in the context of matching to UV-complete models given that  in many BSM scenarios the EWPOs
provide the dominant constraints~\cite{Ellis:2020unq}.
%
The new implementation of EWPOs in {\sc\small SMEFiT} will be discussed in
a separate publication~\cite{ewpos}
and here we provide
for completeness a short summary.

Experimental data and SM predictions
for the legacy EWPOs from LEP and SLAC are taken from~\cite{ALEPH:2005ab}.
%\Jaco{Add info on bhabha}
%
Linear and quadratic SMEFT corrections to these observables arising from dim-6 operators have been computed with {\sc\small mg5\_aMC@NLO} interfaced to SMEFT@NLO.
%
Our implementation of the  EWPOs has been benchmarked by comparing with the results
of~\cite{Brivio:2017bnu}, assuming the same theoretical settings and choice of input dataset. 
%
Specifically, for this benchmarking exercise we use the $m_W$ electroweak input scheme, linear EFT corrections, LO cross-sections, and assume flavour universality.
%
Furthermore, we adopt the same convention on triple gauge operator $O_{WWW}$, which differs from SMEFT@NLO by a negative sign.
%
%
Fig.~\ref{fig:ewpo_benchmark} displays the bounds at the $68\%$ CL for one-parameter fits
in the two studies.
%
Good agreement between our implementation and that of~\cite{Brivio:2017bnu} is obtained for all operators.
%
Residual differences can be explained due to the inclusion of flavour-sensitive observables from LEP which are absent in~\cite{Brivio:2017bnu}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\linewidth]{_inputs/smefit_uv/figures/ewpo_benchmark.pdf}
    \caption{Comparison of a {\sc\small SMEFiT}-based analysis
of the electroweak precision observables from LEP against the corresponding analysis from~\cite{Brivio:2017bnu}
based on the same dataset.
%
We display bounds at the $68\%$ CL for one-parameter fits using linear EFT and LO calculations.
%
In this comparison, we adopt the convention of~\cite{Brivio:2017bnu} for the
triple gauge operator $O_{WWW}$, which differs from the SMEFT@NLO one by a negative sign. 
%
For consistency with the settings
adopted in~\cite{Brivio:2017bnu}, the triple
gauge operator $c_{WWW}$ has been fitted to a subset
of the available LEP data composed by only 4 bins.
}
    \label{fig:ewpo_benchmark}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Taking into account this updated EWPOs
implementation, when compared to the results of~\cite{Ethier:2021bye,Giani:2023gfq} the present global SMEFT analysis used
to constrain UV models
contains
$14$ additional Wilson coefficients $\mathbf{c}$ to be constrained from the fit for a total of 50 independent parameters.
%
The  new degrees of freedom are constrained not only by the EWPOs, but also top quark and diboson measurements.
%
For this reason,
we have recomputed EFT cross-sections for all the processes where such operators are relevant.
%
As in the original analysis~\cite{Ethier:2021bye}, we use {\sc\small mg5\_aMC@NLO}
interfaced to SMEFT@NLO to evaluate linear and quadratic EFT corrections which are augmented with  NLO QCD perturbative corrections whenever available.
%
To avoid overlap between datasets entering the PDF and EFT fits~\cite{Kassabov:2023hbm,Greljo:2021kvv}, we use NNPDF4.0 NNLO no-top~\cite{NNPDF:2021njg} as input PDF set.
%
The values of the input electroweak parameters are taken to be $m_W = 80.387$ GeV, $m_Z =  91.1876$ GeV and $G_F = 1.1663787\cdot 10^{-5}$ $\mathrm{GeV}^{-2}$.
%
Finally, the same flavour assumptions as in~\cite{Ethier:2021bye} are used i.e. a U(2)$_q\times$ U(2)$_u\times $U(3)$_d\times [$U(1)$_\ell\times $U(1)$_e]^3$ symmetry in the quark and lepton sectors. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
    \centering
\includegraphics[width=0.88\linewidth]{_inputs/smefit_uv/figures/bounds_smefit30_vs_smefit20_lin.pdf}
    \caption{The 
    results of the global {\sc\small SMEFiT} analysis, comparing
    the approximated~\cite{Ethier:2021bye,Giani:2023gfq} and exact~\cite{ewpos}
    implementation of the EWPOs.
    %
    For each of the Wilson coefficients entering the fit,
    we indicate the best-fit results and the  marginalised 68\% CL (95\% CL) intervals
    with thicker (thinner) lines.
    %
    The fit labelled as ``Approx EWPOs"
    differs slightly from that of~\cite{Giani:2023gfq}
    due to the use of 
    improved theory predictions, see text
    for more details.
    %
    Operators are grouped by type: from top to bottom, we show two-fermion-two-boson (2F2B),  two-heavy-two-light (2Q2q), four-heavy quarks (4Q), and purely bosonic (B) operators.
    }
    \label{fig:bounds_smefit30_vs_smefit20}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In addition to Fig.~\ref{fig:post_smefit30_vs_smefit20-label},
the impact of the exact implementation of EWPOs 
in the SMEFT fit is also illustrated in Fig.~\ref{fig:bounds_smefit30_vs_smefit20},
which compares the 68\% and 95\% CL
 marginalised bounds on the Wilson coefficients 
 obtained with the approximate
 and exact implementations.
 %
 As mentioned before,
 the results
labelled as ``Approx EWPOs'' differ slightly from 
those in~\cite{Giani:2023gfq} due to the use of improved EFT theory predictions.
%
In general one observes good agreement
between the 
results of the global EFT fit with
approximate and exact 
implementation of the EWPOs, with small
differences whose origin is discussed in~\cite{ewpos}.


==> _inputs/smefit_uv/app-logs.tex <==

The logarithms in one-loop matching expressions such as that of Eq.~(\ref{eq:oneloop_logs_example}) arise as a consequence of the RG running of both the UV couplings and the EFT coefficients.
%
Their appearance ensures that the matching
result is correct irrespective of the choice
of matching scale~\cite{Gherardi:2020det, Carmona:2021xtq}. 
%
In this appendix we revisit this point
in the explicit case of the
heavy scalar model defined by
the Lagrangian of Eq.~\eqref{eq:Lag_UV_full_Varphi_model}. 
%
We start with the general expression, valid for a any
 matching scale $Q$, for the Wilson coefficient $c_{qu,pqrs}^{(8)}$,
which is the most general form in flavour space of the coefficient \cQteight~ generated by this model.
 %
 Subsequently, we evaluate this matching
 relation at two
 different scales, $Q=m_\phi$ and $Q=\mu<m_\phi$, to obtain the results for $c_{qu,pqrs}^{(8)}|_{Q=m_\phi}$ and $c_{qu,pqrs}^{(8)}|_{Q=\mu}$. We expect only the former to be free of RG logarithms.

Then we  use the RGEs for the Wilson
coefficients in the EFT and for the UV couplings of the heavy scalar model to evolve $c_{qu,pqrs}^{(8)}|_{Q=m_\phi}$ down to the scale $\mu$ to obtain $c_{qu,pqrs}^{(8)}|_{Q=m_\phi\to\mu}$. 
%
The comparison between the two calculations, $c_{qu,pqrs}^{(8)}|_{Q=m_\phi\to\mu}$ and $c_{qu,pqrs}^{(8)}|_{Q=\mu}$, will tell us whether the logarithms arising
in the general matching formula correspond to the ones generated by the RG running or not. 
%
This procedure, which was also adopted
in App.~C of~\cite{Carmona:2021xtq}, is sketched in Fig.~\ref{fig:Log_check}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!]
	\centering
		\includegraphics[width=0.9\linewidth]{_inputs/smefit_uv/figures/Logs_sketch.png}  
	\caption{Sketch of the procedure adopted
 to verify the origin of the logarithms
 arising in the one-loop matching formulas.
 %
 The general matching expression for
 the EFT coefficient $c/\Lambda^2$ in terms of UV
 couplings is evaluated at two different scales, $Q=m_{\rm UV}$ and $Q=\mu < m_{\rm UV}$,
 and one verify whether or not the two results
 are entirely related by RGE running.
 }
	\label{fig:Log_check}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For illustration purposes, we perform this check separately at $\mathcal{O}\lp g_3^2\rp $ and then at $\mathcal{O}\lp g_1^2\rp$, i.e. the contributions that depends on the matching scale $Q$ will only be kept at that order. 
%
On the other hand, we perform it without applying any flavour assumption on the EFT coefficient nor the UV model.

\myparagraph{Order $g_3^2$ validation.}
%
The starting point of this calculation
is the general matching result at one-loop for 
the Wilson coefficient $c_{qu,prst}^{(8)}$
in the heavy scalar model, given by
\begin{align}
%\begin{split}
	\frac{c_{qu,prst}^{(8)}}{\Lambda^2}=&-\frac{\big(y_{\phi}^{u}\big)_{pt} \big(y_{\phi}^{u}\big)_{rs}^{*}}{m_\phi^2}-\frac{g_3^2\,\delta_{s,t} \big(y_{\phi}^{d}\big)_{ir} \big(y_{\phi}^{d}\big)_{ip}^{*} }{144 \pi^2\,m_{\phi}^2} \(4-3\log\lp \frac{m_{\phi}^2}{Q^2}\rp \) \nonumber \\  
    &-\frac{g_3^2\,\delta_{p,r} \big(y_{\phi}^{u}\big)_{it} \big(y_{\phi}^{u}\big)_{is}^{*} }{72 \pi^2\,m_{\phi}^2} \(4-3\log\lp \frac{m_{\phi}^2}{Q^2}\rp \) 
    -\frac{g_3^2\,\delta_{s,t} \big(y_{\phi}^{u}\big)_{pi} \big(y_{\phi}^{u}\big)_{ri}^{*} }{144 \pi^2\,m_{\phi}^2} \(4-3\log\lp \frac{m_{\phi}^2}{Q^2}\rp\)\\
    & +\frac{g_3^2 \big(y_{\phi}^{u}\big)_{pt} \big(y_{\phi}^{u}\big)_{rs}^{*} }{48\pi^2 m_\phi^2}+\mcO\(\frac{g_3^0}{16\pi^2}\), \nonumber
%\end{split}
\label{eq:rge_check_cqu8_1loop}
\end{align}
where $prst$ indicate the flavour indices and we omitted the one-loop contributions that do not depend on  the $g_3$ coupling.
%
As expected, all the logarithms appearing
in this expression are removed by setting the matching scale at the heavy scalar mass, $Q=m_\phi$.

The renormalisation group equations 
relevant to describe the scale dependence of this specific Wilscon coefficient are given by~\cite{Alonso:2013hga},
\begin{align}
	\mu\frac{d c_{qu,prst}^{(8)}}{d\mu} = \frac{\beta(c_{qu,prst}^{(8)})}{16\pi^2}= & \frac{g_3^2}{16\pi^2}\left(\frac{4}{3}\delta_{s,t} \( c_{qq,pjjr}^{(1)} + c_{qq,jrpj}^{(1)} \) +4 \delta_{s,t} \(c_{qq,pjjr}^{(3)}+c_{qq,jrpj}^{(3)}\) \right. \nonumber\\
 & +\frac{2}{3}\delta_{s,t} \left(c_{qu,prjj}^{(8)}+c_{qd,prjj}^{(8)}\right) +\frac{4}{3} \delta_{p,r} c_{qu,jjst}^{(8)} +\frac{2}{3} \delta_{p,r} c_{ud,stjj}^{(8)} \\
 &\left. + \frac{4}{3} \delta_{p,r} c_{uu,sjjt} + \frac{4}{3} \delta_{p,r} c_{uu,jtsj} - 14 c_{qu,prst}^{(8)} - 12 c_{qu,prst}^{(1)} \right), \nonumber
\end{align}

\begin{equation}
	\mu\frac{d \big(y_{\phi}^{u}\big)_{pt} }{d\mu}=\frac{\beta\left(\big(y_{\phi}^{u}\big)_{pt}\right)}{16\pi^2}=-\frac{g_3^2}{2\pi^2} \big(y_{\phi}^{u}\big)_{pt},
\end{equation}
\begin{equation}
		\mu\frac{d m_\phi}{d\mu}=0,
\end{equation}
where again we have kept only those terms proportional to $g_3^2$.
%
The RGE equations for the Yukawa
coupling $\big(y_{\phi}^{u}\big)_{pt}$ and the heavy mass $m_\phi$ were computed with {\sc\small RGBeta}~\cite{Thomsen:2021ncy} and cross-checked against 
the results of~\cite{Ferreira:2015rha}.
%
We can solve these RGEs at leading log accuracy to obtain,
\begin{equation}
	c_{qu,prst}^{(8)}\(\mu\)=c_{qu,prst}^{(8)}\(m_\phi\)+\frac{\beta(c_{qu,prst}^{(8)})}{32\pi^2}\log\(\frac{\mu^2}{m_\phi^2}\),
\end{equation}
and similarly for $\big(y_{\phi}^{u}\big)_{pt}$, while $m_\phi$ is constant at this order.
%
The required tree-level matching results are,
\begin{equation}
	c_{qq,ijkl}^{(1)}=c_{qq,ijkl}^{(3)}=c_{ud,ijkl}^{(8)}=c_{uu,ijkl}=0,
\end{equation}
\begin{equation}
	\frac{c_{qd,ijkl}^{(8)}}{\Lambda^2}= -\frac{\big(y_{\phi}^{d}\big)_{kj} \big(y_{\phi}^{d}\big)^{*}_{li}}{m_\phi^2},
\end{equation}
\begin{equation}
	\frac{c_{qu,ijkl}^{(1)}}{\Lambda^2} = -\frac{ \big(y_{\phi}^{u}\big)_{il} \big(y_{\phi}^{u}\big)^{*}_{jk} }{6\, m_\phi^2},
\end{equation}
which substituting in the corresponding
beta function allows one to compute $\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=\mu}$ as,
\begin{align}
\label{appD:eqC9}
%\begin{split}	
\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=\mu}= &\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=m_{\phi}} +  \frac{\beta(c_{qu,prst}^{(8)})}{32\pi^2\Lambda^2}\log\(\frac{\mu^2}{m_\phi^2}\),\nonumber\\
= & \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm tree},Q=m_{\phi}}+\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{ { \rm loop},Q=m_{\phi}}+  \frac{\beta(c_{qu,prst}^{(8)})}{32\pi^2\Lambda^2}\log\(\frac{\mu^2}{m_\phi^2}\),
%\end{split}
\end{align}
where we have defined
\begin{equation}
	\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm loop},Q=m_{\phi}}= -\frac{g_3^2\,\delta_{s,t} \big(y_{\phi}^{d}\big)_{ir} \big( y_{\phi}^{d} \big)^{*}_{ip} }{36 \pi^2\,m_{\phi}^2} 
	-\frac{g_3^2\,\delta_{p,r} \big( y_{\phi}^{u} \big)_{it} \big( y_{\phi}^{u} \big)^{*}_{is} }{18 \pi^2\,m_{\phi}^2}
	-\frac{g_3^2\,\delta_{s,t} \big( y_{\phi}^{u} \big)_{pi} \big( y_{\phi}^{u} \big)^{*}_{ri} }{36 \pi^2\,m_{\phi}^2} + \frac{g_3^2 \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u}\big)^{*}_{rs} }{48\pi^2 m_\phi^2}.
\end{equation}
The last term in Eq.~(\ref{appD:eqC9})
is the contribution related
to the running between $Q=m_\phi$
and $Q=\mu<m_{\phi}$.

To keep everything consistently at leading-log and one-loop order, all the couplings in the previous expression should be considered as constant with energy, and hence $\lp c_{qu,prst}^{(8)}/\Lambda^2\rp\Big|_{{\rm loop},Q=m_{\phi}}$ is equal to  $\lp c_{qu,prst}^{(8)}/\Lambda^2\rp \Big|_{{\rm loop},Q=\mu}$ except for the logarithmic pieces. The same is not true for the tree-level contribution, which has to be transformed as follows.
\begin{align}
	\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{tree,Q=m_{\phi}} =& -\frac{ \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs} }{m_\phi^2}\Big|_{Q=m_\phi} = -\frac{ \big( y_{\phi}^{u}(m_\phi) \big)_{pt} \big( y_{\phi}^{u}(m_\phi) \big)_{rs}^{*} }{m_\phi^2} \nonumber\\
	=&-\frac{\( \big(y_{\phi}^{u}(\mu)\big)_{pt} - \frac{ \beta\Big(\big(y_{\phi}^{u}\big)_{pt}\Big)}{32\pi^2}\log(\frac{\mu^2}{m_\phi^2})\) \( \big(y_{\phi}^{u}(\mu)\big)_{rs} - \frac{\beta\Big(\big(y_{\phi}^{u}\big)_{rs}\Big)}{32\pi^2}\log(\frac{\mu^2}{m_\phi^2}) \)^{*} }{m_\phi^2 } \nonumber \\
	=&-\frac{\big(y_{\phi}^{u}\big)_{pt} \big(y_{\phi}^{u}\big)^{*}_{rs} }{m_\phi^2}\Big|_{Q=\mu}+\frac{\beta\Big( \big( y_{\phi}^{u} \big)_{pt} \Big) \big( y_{\phi}^{u} \big)^{*}_{rs} }{32\pi^2\,m_{\phi}^2}\log\lp \frac{\mu^2}{m_\phi^2}\rp  +\frac{ \big( y_{\phi}^{u} \big)_{pt} \beta\Big( \big(y_{\phi}^{u}\big)_{rs} \Big)^{*} }{ 32 \pi^2 \, m_{\phi}^2}\log\lp \frac{\mu^2}{m_\phi^2}\rp,
\end{align}
where in the first two lines we indicate explicitly the scale at which the UV couplings are evaluated and in the last line we have kept only the leading log terms. The first term in the last line can be identified as $\lp c_{qu,prst}^{(8)}/\Lambda^2\rp \Big|_{{\rm tree},Q=\mu}$.
Hence, now we have,
\begin{equation}
	\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=\mu}= \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{tree,Q=\mu}+\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm loop},Q=m_{\phi}} +\frac{ \beta\Big( \big( y_{\phi}^{u} \big)_{pt} \Big) \big( y_{\phi}^{u} \big)^{*}_{rs} + \big( y_{\phi}^{u} \big)_{pt} \beta\Big( \big( y_{\phi}^{u} \big)_{rs} \Big)^{*} +\beta( c_{qu,prst}^{(8)})}{32\pi^2\,m_{\phi}^2}\log\lp \frac{\mu^2}{m_\phi^2}\rp.
 \nonumber
\end{equation}
Finally, one has to replace the expressions for the $\beta$ functions computed before, use the tree-level matching results inside the $\beta$ function for the Wilson coefficient, and reorder the terms. This leads to Eq.~\eqref{eq:rge_check_cqu8_1loop} evaluated at $Q=\mu$, concluding the check.

\myparagraph{Order $g_1^2$ validation.}
%
Next we perform the same check at order $g_1^2$.
The general matching result at 1-loop for $c_{qu,prst}^{(8)}$ is
\begin{equation}
	\begin{split}
		\frac{c_{qu,prst}^{(8)}}{\Lambda^2}=-\frac{\big(y_{\phi}^{u}\big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs} }{m_\phi^2} -\frac{25 g_1^2 \big( y_{\phi}^{u} \big)_{pt} \big(y_{\phi}^{u}\big)^{*}_{rs}  }{ 1152 \pi^2 m_{\phi}^{2} } + \mcO\(\frac{g_1^0}{16\pi^2}\),
	\end{split}
 \label{eq:rge_check_cqu8_g1}
\end{equation}
where the omitted terms are 1-loop contributions that do not depend on $g_1$. In this case, there are no logarithms in the expression. Hence, the only terms that have a dependence on the energy scale are the ones generated at tree-level.

The RGE equations we need are in this case are~\cite{Alonso:2013hga,Ferreira:2015rha},
\begin{equation}
	\begin{split}
		\mu\frac{d c_{qu,prst}^{(8)}}{d\mu} =\frac{\beta(c_{qu,prst}^{(8)})}{16\pi^2}=-\frac{g_1^2}{12\pi^2}c_{qu,prst}^{(8)},
	\end{split}
\end{equation}
\begin{equation}
	\begin{split}
		\mu\frac{d \big(y_{\phi}^{u}\big)_{pt}}{d\mu}=\frac{\beta\Big(\big(y_{\phi}^{u}\big)_{pt} \Big) }{16\pi^2}=-\frac{ 17 g_1^2}{192\pi^2} \big( y_{\phi}^{u} \big)_{pt},
	\end{split}
\end{equation}
\begin{equation}
		\mu\frac{d m_\phi}{d\mu}= \frac{\beta(m_{\phi})}{16\pi^2} = -\frac{3g_1^2}{64\pi^2} m_{\phi},
\end{equation}
where we have kept only those terms proportional to $g_1^2$.
The leading-log solution reads,
\begin{equation}
	c_{qu,prst}^{(8)}\(\mu\)=c_{qu,prst}^{(8)}\(m_\phi\)+\frac{\beta(c_{qu,prst}^{(8)})}{32\pi^2} \log\(\frac{\mu^2}{m_\phi^2}\),
\end{equation}
\begin{equation}
	m^2_{\phi}\(m_\phi\)=m^2_{\phi}\( \mu \)- m_{\phi}\(\mu\)\frac{\beta(m_{\phi})}{16\pi^2} \log\(\frac{\mu^2}{m_\phi^2}\),
\end{equation}
and analogously for the UV coupling.

All the required tree-level matching results were shown in the previous subsection. We can compute $\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=\mu}$ as,
\begin{align}
%	\begin{split}	
		\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=\mu} &= \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=m_{\phi}} + 
		\frac{\beta(c_{qu,prst}^{(8)})}{32\pi^2\Lambda^2}\log\(\frac{\mu^2}{m_\phi^2}\),\nonumber\\
		&= \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm tree},Q=m_{\phi}} + \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm loop},Q=m_{\phi}} +  \frac{\beta(c_{qu,prst}^{(8)})}{32\pi^2\Lambda^2}\log\(\frac{\mu^2}{m_\phi^2}\),
%	\end{split}
\end{align}
where
\begin{equation}
	\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{loop,Q=m_{\phi}}= -\frac{25 g_1^2 \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs}  }{ 1152 \pi^2 m_{\phi}^{2} }.
\end{equation}
Let us remark again that all the UV couplings in $\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm loop},Q=m_{\phi}}$ should be considered as constant with energy. 
The tree-level contribution at the two different scales are related as,
%\begin{equation}
	\begin{align}
		\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{tree,Q=m_{\phi}} &= -\frac{ \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs} }{m_\phi^2}\Big|_{Q=m_\phi} = -\frac{\big( y_{\phi}^{u}(m_\phi)\big)_{pt} \big(y_{\phi}^{u}(m_\phi) \big)^{*}_{rs} }{m_\phi^2} \nonumber\\
		&=-\frac{ \( \big( y_{\phi}^{u}(\mu) \big)_{pt} - \frac{\beta\Big( \big(y_{\phi}^{u} \big)_{pt} \Big) }{32\pi^2}\log(\frac{\mu^2}{m_\phi^2})\) \( \big( y_{\phi}^{u}(\mu) \big)_{rs} - \frac{\beta\Big( \big( y_{\phi}^{u} \big)_{rs} \Big)}{32\pi^2}\log(\frac{\mu^2}{m_\phi^2}) \)^{*} }{ m^2_{\phi}\( \mu \)- m_{\phi}\(\mu\)\frac{\beta(m_{\phi})}{16\pi^2} \log\(\frac{\mu^2}{m_\phi^2}\) } \nonumber\\
		&=-\frac{ \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs} }{m_\phi^2}\Big|_{Q=\mu}+\frac{\beta\Big( \big( y_{\phi}^{u}\big)_{pt}\Big) \big( y_{\phi}^{u} \big)^{*}_{rs} +\big( y_{\phi}^{u} \big)_{pt} \beta\Big( \big(y_{\phi}^{u}\big)_{rs} \Big)^* }{ 32\pi^2\,m_{\phi}^2 }\log(\frac{\mu^2}{m_\phi^2}) \nonumber\\
   &\phantom{=} - \frac{ \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs} }{ m_\phi^2} \frac{\beta(m_{\phi})}{16\pi^2 m_{\phi}} \log\(\frac{\mu^2}{m_\phi^2}\),
	\end{align}
%\end{equation}
where we have kept only the leading-log terms. The first term in the last line is $\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm tree},Q=\mu}$.

Hence, in total we have,
\begin{align}
	\frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{Q=\mu} =& \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm tree},Q=\mu} + \frac{c_{qu,prst}^{(8)}}{\Lambda^2}\Big|_{{\rm loop},Q=m_{\phi}}\nonumber\\
	&+\frac{\beta\Big(\big(y_{\phi}^{u}\big)_{pt}\Big) \big(y_{\phi}^{u}\big)^{*}_{rs} + \big(y_{\phi}^{u}\big)_{pt} \beta\Big( \big( y_{\phi}^{u} \big)_{rs} \Big)^{*} - 2 \tfrac{\beta(m_{\phi})}{m_\phi} \big( y_{\phi}^{u} \big)_{pt} \big( y_{\phi}^{u} \big)^{*}_{rs}  +\frac{m_\phi^2}{ \Lambda^2}\beta(c_{qu,prst}^{(8)})}{32\pi^2\,m_{\phi}^2}\log\lp \frac{\mu^2}{m_\phi^2}\rp \, . \nonumber
\end{align}
Replacing the $\beta$ functions computed before and reordering, one finds that the logarithmic term vanishes exactly, in perfect agreement with Eq.~\eqref{eq:rge_check_cqu8_g1}. 

Finally, let us remark the key role played by the RGEs of the UV variables, $y_{\phi}^{u}$ and $m_{\phi}$, in both checks at order $g_3^2$ and $g_1^2$. Had we not considered them, there would have been residual logarithmic effects not accounted for by the RGEs, as found in~\cite{Brivio:2021alv}. The same checks can be performed with other WCs and at all orders in the couplings.

==> _inputs/smefit_uv/app-mmeft.tex <==
\section{The {\sc match2fit}~package}
\label{app:mmeft2smefit}
\label{app:mmeft2smefit-conceptual-description}

As mentioned in the introduction,
several public tools to carry out
global analyses of experimental data
in the SMEFT framework have been presented.
%
Some of these tools also include the
option to carry out parameter scans
in the space of pre-defined UV models matched to SMEFT. 
%
While the matching procedure
between UV models and the SMEFT coefficients has been automated at tree-level and partially at 1-loop level, currently 
there is no streamlined method enabling
the interface of the
output of these matching codes with
SMEFT fitting frameworks.
%
Such interface would allow  
using the SMEFT to impose bounds on the
parameter space of general, user-defined
UV-complete models.

In this appendix we describe
the {\sc\small match2fit}~package used in this work
to interface an EFT automated matching code,
specifically {\sc\small MatchMakerEFT}, with
a global fitting analysis framework, in this  case
{\sc\small SMEFiT}.
%
The current public version of this package is available on \href{https://github.com/arossia94/match2fit}{ Github~\faicon{github} }.
%
We emphasise that the novel functionality of \matchTOfit~is the automated translation of matching results between the formats used by the matching and fitting codes.
%
This could be extended to connect different SMEFT-related codes. 
%
We provide here a succinct introduction
to this code, and point
the interested reader to the 
\href{https://github.com/arossia94/match2fit/blob/main/match2fit_Users_Manual.pdf}{user's manual}
for more details.

The package has two different working modes. 
%
The first one reads the matching output in the format used by {\sc\small MatchMakerEFT}~and parses it to the format of run cards that can be fed into \smefit.
%
In this mode, the mandatory inputs are the location of the file containing the matching results and a numerical value (in TeV) for the mass of the heavy particle. 
%
Optionally, one can also specify a name for the UV model and define a ``collection'', 
a set of UV models with common characteristics. 
%
Depending on the executed function, the code will print the run card for a scan on the UV parameters with or without the accompanying file that defines the UV invariants (see Sect.~\ref{sec:uv_invariants}).

The second mode combines the first one with a wrapper for {\sc\small MatchMakerEFT}~to perform the matching of a given UV model to SMEFT. 
%
This model allows the user to go from the files that define the UV model to the run cards for \smefit~in a single command.
%
It is also possible to just perform the matching without producing the run cards for SMEFiT.
%
The input required in this mode is the one that {\sc\small MatchMakerEFT}~needs to describe the heavy particles that will be integrated out.  More precisely, it needs the \verb|.fr|, \verb|.red| and \verb|.gauge| files, and optionally the \verb|.red| file. The \verb|.fr| file is just a FeynRules file that defines the heavy particle(s), its (their) free Lagrangian and its (their) interactions with the SM. 
%
The SM and SMEFT models are included in {\sc\small MatchMakerEFT}~and can be used
in this context without further modification. 
%
See~\cite{Carmona:2021xtq} for more details on how to write the \verb|.fr| file and what the other files must contain.

The {\sc\small match2fit} code consists of
a Wolfram Mathematica Package designed and tested in version $12.1$ or later. 
%
To unlock its full functionality, this package requires a working installation of {\sc\small MatchMakerEFT}.



\myparagraph{Main commands.}

In order to highlight its usage, we 
describe now the key commands
made available by the {\sc\small match2fit}
package. 


\begin{itemize}

\item {\lstinline[emph={directory,model}]|parametersList[directory,model]|}: Both arguments should be strings. This function reads the file \verb|model.fr| in \verb|directory|, recognizes the masses and couplings of the heavy particles to be integrated out, and gives back an array with two elements. 
%
The first element is a list with the symbolical expression of the masses of the heavy particles. The second element is a list of the couplings defined for these heavy particles, excluding gauge couplings but not self-interactions.
    
\item {\lstinline[emph={matchResFile,looplevel}]|parametersListFromMatchingResult[matchResFile,looplevel]|}: Its first argument must be a string with the address of the file containing the matching results. It recognizes the masses and couplings of the heavy particles from those results and gives an output in the same format as \lstinline|parametersList|. This code assumes that any parameter with a name starting by \textit{m} or \textit{M} corresponds to a mass and identifies any other parameter as a coupling. If the input of \lstinline|parametersListFromMatchingResult| is the matching result obtained with the model fed into \lstinline|parametersList|, any difference in their outputs should be due to couplings (or whole particles) that do not affect the tree-level matching result. If the second argument, \lstinline|looplevel|, is equal to \lstinline|0|, \lstinline|"tree"|, or \lstinline|"Tree"|, and the input file contains 1-loop matching results, the 1-loop contributions will be ignored. To use 1-loop results, \lstinline|looplevel| must be set to \lstinline|1|, \lstinline|"loop"|, or \lstinline|"1loop"|. If the input file corresponds to tree-level matching results, there might be some spurious 1-loop pieces due to evanescent shifts (see \href{https://gitlab.com/m4103/matchmaker - eft/-/issues/12}{here}) and hence \lstinline|looplevel| must be set to \lstinline|0|, \lstinline|"tree"|, or \lstinline|"Tree"| to ensure their consistent removal.

\item {\lstinline[emph={matchResFile}]|flavourSymChecker[matchResFile,Options]|}: It takes the file with matching results specified as input and checks if those results are compatible with the \smefit~flavour symmetry, U$(2)_{q}\times$U$(2)_{u}\times$U$(3)_{d}\times(\text{U}(1)_{\ell}\times\text{U}(1)_{e})^3$. If the constraints are satisfied, it returns YES. If not, it returns NO and it prints the first WC for which it found a symmetry violation. The option \lstinline|"UVFlavourAssumption"| allows the user to specify a replacement list that can be used to apply flavour assumptions on the UV parameters. The left-hand side of the replacement rule should contain some of the UV parameters listed by \lstinline|parametersListFromMatchingResult| or \lstinline|parametersList| with or without numerical indices, according to how they appear in the matching results file. The code supports up to 4 numerical indices in a single group, i.e. couplings such as gUV, gUV$[1]$, gUV$[1,3]$ and gUV$[1,3,2,4]$ are supported, but gUV$[1][3]$ or gUV$[1][2,3]$ are not. The default value of \lstinline|"UVFlavourAssumption"| is an empty list. An example of how to set this option is,
\begin{lstlisting}
{"UVFlavourAssumption" -> {gWtiQ[i_, j_] :> KroneckerDelta[i,j] * KroneckerDelta[i, 3] gWqf[3, 3] }}
\end{lstlisting}
This function is prepared to handle tree-level matching results only. If it detects 1-loop results in the input file, it warns the user of its limitations and proceeds to ignore the 1-loop contributions. Some models matched at tree-level might trigger the warning due to the presence of spurious 1-loop pieces related to the evanescent shifts (see \href{https://gitlab.com/m4103/matchmaker - eft/-/issues/12}{here}) which are consistently ignored by this function.

\item {\lstinline[emph={matchResFile}]|flavourSolver[matchResFile, Options]|}: It takes the file with matching results specified as input and tries to solve the constraints imposed by the \smefit~flavour symmetry, U$(2)_{q}\times$U$(2)_{u}\times$U$(3)_{d}\times(\text{U}(1)_{\ell}\times\text{U}(1)_{e})^3$, for the UV couplings. The running time, the number of solutions and their complexity depend on the model. It returns all found solutions. The only Option of this function is \lstinline|"UVFlavourAssumption"|, which follows the same description given in the function \lstinline|flavourSymChecker|. This function considers the SM Yukawa couplings as symbolical variables and they can be set to zero with the option \lstinline|"UVFlavourAssumption"|. As with \lstinline|flavourSymChecker|, this function is prepared to handle tree-level matching results only.

\item {\lstinline[emph={directory, model, looplevel}]|matcher[directory, model, looplevel]|}: it runs {\sc\small MatchMakerEFT}~and performs the tree-level matching without printing any run card for \smefit. It takes two strings as arguments, \emph{\lstinline|directory|} and \emph{\lstinline|model|}. The first one is the directory where the package will look for the files \verb|model.fr|, \verb|model.red| and \verb|model.gauge|. If the code does not find one of those files, it will print a warning. It does not check for the existence of \verb|model.herm|. The expected content of each of those files is specified in the documentation of {\sc\small MatchMakerEFT} \cite{Carmona:2021xtq}. The argument \lstinline|looplevel| decides the matching order, \lstinline|looplevel| equal to \lstinline|0|, \lstinline|"tree"|, or \lstinline|"Tree"| will produce tree-level matching, while setting it to \lstinline|1|, \lstinline|"loop"|, or \lstinline|"1loop"| will produce 1-loop level matching. {\sc\small MatchMakerEFT}~will create the folder \verb|directory/model_MM|, inside which the matching results will be stored as \verb|MatchingResult.dat|. The code will check if {\sc\small MatchMakerEFT}~reported any problem during the matching and will print a warning if so. After performing the matching, the package will remove most of the files and directories created by itself or {\sc\small MatchMakerEFT}~for the sake of tidiness. It will only leave the directory \verb|model_MM| and 2 files inside: \verb|MatchingResult.dat| and \verb|MatchingProblems.dat|.

\item{\lstinline[emph={matchResFile, mass, looplevel}]|matchResToUVscanCard[matchResFile,mass, looplevel, Options]|}: Function that reads the file with the tree-level matching results and prints the cards required for a UV scan. \emph{\lstinline|matchResFile|} must be a string with the exact address of the file that contains the matching results to be used. The format of that file should be exactly like the file \verb|MatchingResult.dat| produced by {\sc\small MatchMakerEFT}. The argument \emph{\lstinline|mass|} should be the value in TeV that the mass(es) of the UV particle(s) will be set to. \emph{\lstinline|mass|} can be one numerical value or a list of them \emph{$\lbrace m_1, ..,m_N\rbrace$}, the latter being useful in the case of a multiparticle model. The order of the masses is the one returned by \lstinline|parametersListFromMatchingResult|. If the user specifies only one numerical mass value for a multiparticle model, all the particles will be assigned the same mass. If \lstinline|parametersListFromMatchingResult| identifies $K$ masses and $N<K$, the code will assume  $m_i = m_N$ for $ N \leqslant i \leqslant K$. If $N>K$, the values $m_i$ with $K<i\leqslant N$ will be ignored.
The mass values are also printed on the card names and inside the cards. For multiple masses, the convention is to take the integer part of each value and stick them together in sequence. The third argument is \emph{\lstinline|looplevel|}, which indicates the loop order of the matching results to be parsed and it works as in \lstinline|parametersListFromMatchingResult|. When \emph{\lstinline|looplevel|} is set to \lstinline|1|, \lstinline|loop| or \lstinline|1loop|, the code chooses the matching scale as the minimum of the masses of the UV particles.
There are 3 options. The first one is \lstinline|"UVFlavourAssumption"|, which is identical to the one of the function \lstinline|flavourSymChecker|, see its description for details on this option.
The second option is \lstinline|"Collection"|, a string indicating the Collection to which the model belongs. Its default value is \lstinline|"UserCollection"|. Finally, the option \lstinline|"Model"| is a string that specifies the model name to be printed on the run cards, with default value \verb|"UserModel"|. An example of how to set these options is replacing the argument \lstinline|Options| by:

\begin{lstlisting}
{"UVFlavourAssumption" -> {lambdaT1[a_] :> lambdaT1[3]}, 
 "Collection" -> "TestMatchingCollection","Model"->"TestModel"}
\end{lstlisting}


\end{itemize}

The package also includes a function that integrates the steps of matching and printing all the run cards according to the result of said matching:

\begin{itemize}
    
\item {\lstinline[emph={directory, model, mass, looplevel}]|modelToUVscanCard[directory,model, mass, looplevel, Options]|}: Function that takes the files that define the UV model, performs the tree-level matching by running {\sc\small MatchMakerEFT}, and prints the run cards needed for a UV scan. The first two arguments are exactly like in \verb|matcher|, i.e. the program will look for the files \verb|model.fr|, \verb|model.red|, and \verb|model.gauge| in \verb|directory| and will do the tree-level matching based on them. The argument \verb|model| also defines the name of the model. \verb|mass| should be the value(s) in TeV that the mass(es) of the UV particle(s) will be set to. The handling of several mass values is equal to the function {\lstinline|matchResToUVscanCard|}. The argument \lstinline|looplevel| indicates the loop order at which the matching will be performed and that will be considered when printing the run cards. Its allowed values are as for previous functions. When \emph{\lstinline|looplevel|} is set to \lstinline|1|, \lstinline|loop| or \lstinline|1loop|, the code chooses the matching scale as the minimum of the masses of the UV particles. This function has 2 options. The first one is \lstinline|"UVFlavourAssumption"|, which is identical to the one of the function \lstinline|flavourSymChecker|, see its description for details on this option.
The second option is \lstinline|"Collection"|, a string indicating the Collection to which the model belongs. Its default value is \lstinline|"UserCollection"|. An example of how to set these options is replacing the argument \lstinline|Options| by:

\begin{lstlisting}
{"UVFlavourAssumption" -> {lambdaT1[a_] :> lambdaT1[3]}, 
 "Collection" -> "TestMatchingCollection"}
\end{lstlisting}

\end{itemize}

\myparagraph{Limitations and outlook.}
%\label{app:mmeft2smefit-outlook}
%
In its current incarnation, all SM couplings are numerically evaluated when printing the run cards 
used as input in the global SMEFT fit. 
%
Their values are hard-coded in the package and summarised in App.~A of the {\sc\small match2fit}  user manual.
%
Future versions of {\sc match2fit} should allow the user to vary easily these values.

Another restriction of {\sc match2fit}
is that it does not check for the fulfilment of the \smefit~flavour assumptions automatically when printing the run cards for \smefit. This generates a degree of arbitrariness, e.g. the code uses the matching result for $(c_{\varphi q}^{(3)})_{22}$ as the result for $(c_{\varphi q}^{(3)})_{ii}$ without verifying first that that $(c_{\varphi q}^{(3)})_{22}=(c_{\varphi q}^{(3)})_{11}$.
%
We summarise these choices in App.~B of the user manual. 
%
The user should be aware of this limitation and compensate for it with the required assumptions on the UV couplings.
%
Support for alternative flavour structures on the Wilson coefficients will be added in the future,
to ensure full compatibility with updated versions of the \smefit~analysis and/or becoming compatible with other fitting codes.

We also note that {\sc match2fit}
assumes that all UV couplings are real and applies this assumption when interpreting the matching results. The support for complex UV couplings (and hence also of the corresponding WCs) will be added in future releases.

In the long term, {\sc match2fit} could
be extended to process matching results
provided in the WCxf format~\cite{Aebischer:2017ugx}.
%
This would facilitate the interface with other SMEFT matching codes such as {\sc\small CoDEx} and {\sc\small Matchete} as well as with codes implementing the Renormalisation Group Equations (RGEs) running of SMEFT operators. 

Since version \verb|1.8|, the pipeline required to perform the fit of the UV model matched to the SMEFT at 1-loop level is fully automated. However, accessory functions that might help to analyse the fit results, in particular the one that computes the UV invariants, remain limited to tree-level results. They will support 1-loop results in the future.

==> _inputs/smefit_uv/tables/table_1l_var_m.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.5}\begin{tabular}{c|c|c|c|c|c}
Model & UV invariants & LO $\mathcal{O}\left(\Lambda^{-2}\right)$ &LO $\mathcal{O}\left(\Lambda^{-4}\right)$ & NLO $\mathcal{O}\left(\Lambda^{-2}\right)$ & NLO $\mathcal{O}\left(\Lambda^{-4}\right)$ \\
\toprule
\multirow{3}{*}{$\phi$} & $\left|\lambda_{\phi}\right|$ & $\times$ & $\times$ & $\times$ & $\times$ \\
 & $\mathrm{sgn}(\lambda_{\phi})\left(y_{\phi}^u\right)_{33}$ & [-2.877$\mathrm{e}{1}$, 2.477$\mathrm{e}{1}$] & [-2.471$\mathrm{e}{1}$, 2.106$\mathrm{e}{1}$] & [-2.514$\mathrm{e}{1}$, 2.421$\mathrm{e}{1}$] & [-2.546$\mathrm{e}{1}$, 2.146$\mathrm{e}{1}$]  \\
 & $\left|m_\phi\right|$ & $[45.80, \infty)\GeV$ & $[45.60, \infty)\GeV$ & $[42.98, \infty)\GeV$& $[45.43, \infty)\GeV$ \\
\bottomrule
\end{tabular}
\caption{
Same as the bottom part
of Table~\ref{tab:cl-phi},
now for the case in which the heavy scalar
mass $m_\phi$ is also treated as a free
parameters in the fit based on one-loop
matching conditions.
%
The corresponding posterior distributions
for the three UV invariants
are shown in Fig.~\ref{fig:var-m-post}.
}
\label{tab:cl-1loop-varm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> _inputs/smefit_uv/tables/table_vfermion.tex <==
\begin{table}
\begin{center}
\scriptsize
\renewcommand{\arraystretch}{1.4}\begin{tabular}{c|c|c|c|c|c}
Model & UV invariants & LO $\mathcal{O}\left(\Lambda^{-2}\right)$ &LO $\mathcal{O}\left(\Lambda^{-4}\right)$ & NLO $\mathcal{O}\left(\Lambda^{-2}\right)$ & NLO $\mathcal{O}\left(\Lambda^{-4}\right)$ \\
\toprule
$N$ & $\left|\left(\lambda_N^e\right)_3\right|$ & 0.463 & 0.470 & 0.477 & 0.469 \\
$E$ & $\left|\left(\lambda_E\right)_3\right|$ & 0.250 & 0.248 & 0.245 & 0.242 \\
$\Delta_1$ & $\left|\left(\lambda_{\Delta_1}\right)_3\right|$ & 0.209 & 0.205 & 0.209 & 0.209 \\
$\Delta_3$ & $\left|\left(\lambda_{\Delta_3}\right)_3\right|$ & 0.268 & 0.266 & 0.264 & 0.263 \\
$\Sigma$ & $\left|\left(\lambda_{\Sigma}\right)_3\right|$ & 0.284 & 0.283 & 0.289 & 0.285 \\
$\Sigma_1$ & $\left|\left(\lambda_{\Sigma_1}\right)_3\right|$ & 0.423 & 0.424 & 0.432 & 0.421 \\
$U$ & $\left|\left(\lambda_{U}\right)_3\right|$ & 0.845 & 0.857 & 0.824 & 0.853 \\
$D$ & $\left|\left(\lambda_{D}\right)_3\right|$ & 0.230 & 0.230 & 0.233 & 0.228 \\
$Q_1$ & $\left|\left(\lambda_{\mathcal{Q}_1}^u\right)_3\right|$ & 0.943 & 0.929 & 0.913 & 0.937 \\
$Q_7$ & $\left|\left(\lambda_{\mathcal{Q}_7}\right)_3\right|$ & 0.937 & 0.908 & 0.919 & 0.908 \\
$T_1$ & $\left|\left(\lambda_{T_1}\right)_3\right|$ & 0.470 & 0.451 & 0.454 & 0.450 \\
$T_2$ & $\left|\left(\lambda_{T_2}\right)_3\right|$ & 0.387 & 0.376 & 0.375 & 0.386 \\
\bottomrule
\end{tabular}
\caption{95\% CI of the heavy vector fermion fields UV couplings.}
\end{center}
\end{table}

